Compact Optimality Verification for Optimization Proxies

Recent years have witnessed increasing interest in optimization proxies, i.e., machine learning models that approximate the input-output mapping of parametric optimization problems and return near-optimal feasible solutions. Following recent work by (Nellikkath & Chatzivasileiadis, 2021), this paper reconsiders the optimality verification problem for optimization proxies, i.e., the determination of the worst-case optimality gap over the instance distribution. The paper proposes a compact formulation for optimality verification and a gradient-based primal heuristic that brings substantial computational benefits to the original formulation. The compact formulation is also more general and applies to non-convex optimization problems. The benefits of the compact formulation are demonstrated on large-scale DC Optimal Power Flow and knapsack problems.

==> tex_rebuttal/results.tex <==
\section{Numerical Results}
\label{sec:results}

\subsection{Optimality Verification for DCOPF}
\label{sec:results:DCOPF}

\subsubsection{Experiment Setup}
The optimality verification for DCOPF proxies is evaluated over IEEE 57-/118-/300-bus and Pegase 1354-bus test cases from the PGLib library \cite{babaeinejadsarookolaee2019power}.
The data generation follows \cite{chen2023end}.
Denote by $\vd^{\text{ref}}$ the nodal load vector from the reference PGLib case.
The instances are generated by perturbing the reference load vector.
Namely, for instance $i$, $\vd^{(i)} = (\gamma^{(i)}+ \boldsymbol{\eta^{(i)}})\times\vd^{\text{ref}}$, 
where $\gamma^{(i)} \in \sR$ is a global scaling factor and $\boldsymbol{\eta^{(i)}}\in \mathbb{R}^{B}$ denotes element-wise noises.
The $\gamma$ is sample from uniform distribution $U[80\%, 120\%]$ and for each load, $\eta$ is sampled from a uniform distribution $U[-5\%, 5\%]$.
For every test case, $50,000$ instances are generated and solved for training.
The optimization proxies are trained using the self-supervised learning algorithm in \cite{chen2023end}, which is detailed in the Appendix \ref{appendix:dcopf:training}.

To generate the optimity verification instances, the input domain is defined as a hyperhexagon for the optimization proxies:
\begin{align*}
    &\gX = \{(\alpha + \mBeta)\cdot \vd^{\text{ref}}| 1 - u \leq \alpha \leq 1 + u, \mathbf{-5\%} \leq \mBeta \leq \mathbf{5\%}\},
\end{align*}
where $\alpha \in \sR$, $\mBeta \in \sR^{B}$ and $u$ control the size of the input domains.

To accelerate the optimization solving, PGA-VFA in Algorithm \ref{alg:pgd} is used as the primal heuristic to find high-quality feasible solutions, where the optimal dual solutions of the $50,000$ instances are used to construct the value function approximation. PGA-VFA is running with 200 threads in parallel with the improvement techniques in Section \ref{sec:improve_techniques}, where the input space is evenly partitioned on $\alpha$ and the initial points are randomly sampled from the vertex of the hyperhexagon. When running PGA-VFA the initial step size is $1e-3$ and is reduced by a factor of then if it cannot find a better primal solution for a consecutive of 10 iterations.
In addition, the PGA-VFA stops if the primal solution does not improve for consecutive 20 iterations or reach the maximum iterations $500$.

To improve the MILP relaxation, this work uses optimization-based bound tightening (OBBT) \cite{caprara2010global} to tighten the variable domain before the ReLU operators, which is detailed in the Appendix \ref{appendix:dcopf:obbt}. To tradeoff the efficiency of bound propagation, Interval Bound Propagation (IBP) \cite{tjeng2017evaluating} is used to tighten the variable domain in the feasibility repair steps.

All verification instances are solved with Gurobi 11.0 \cite{gurobi} with 16 threads and default parameter setting with a time limit of 6 hours. Since the performance of Gurobi varies on different seeds, this experiments solve all instances with 5 different seeds and report value in the shifted geometric means:
\[\mu(x_1, \cdots, x_n) = \exp(\frac{1}{n}\sum_i \log(x_i+s))-s.\]
The paper uses a shift $s$ of 1\% for optimality gaps and 1 for other values.
Experiments are conducted on dual Intel Xeon 6226@2.7GHz machines running Linux on the cluster.

% \subsubsection{Performance of Primal Heuristics}
% \begin{figure*}
%     \centering
%     \subfloat[57 IEEE]{
%         \includegraphics[width=0.48\columnwidth]{figs/BestObjVal_vs_perturbation/objval_perb_57_ieee_hexagon_32.png}
%         \label{fig:ub:DCOPF:57_ieee}
%     }
%     \subfloat[118 IEEE]{
%         \includegraphics[width=0.48\columnwidth]{figs/BestObjVal_vs_perturbation/objval_perb_118_ieee_hexagon_32.png}
%         \label{fig:ub:DCOPF:118_ieee}
%     }
%     \subfloat[300 IEEE]{
%         \includegraphics[width=0.48\columnwidth]{figs/BestObjVal_vs_perturbation/objval_perb_300_ieee_hexagon_32.png}
%         \label{fig:ub:DCOPF:300_ieee}
%     }
%     \subfloat[1354 Pegase]{
%         \includegraphics[width=0.48\columnwidth]{figs/BestObjVal_vs_perturbation/objval_perb_1354_pegase_hexagon_32.png}
%         \label{fig:ub:DCOPF:1354_pegase}
%     }\\
%     \caption{Best objective value of different optimization methods on continuous optimization proxies instances}
%     \label{fig:ub:DCOPF}
% \end{figure*}


\subsubsection{Performance of Exact Verification}
\begin{table}[!t]
    \centering
    \caption{Solving time (s) of Bilevel formulation \cite{nellikkath2021physics} and our Compact formulation on closed instances that can be solved to optimality. Both formulations are warm-started with nominal solutions and solved using Gurobi with the same time limit. The \textcolor{red}{dual} bounds are tightened using OBBT. For a comparison to \textcolor{blue}{open (unsolved)} instances, see Table \ref{tab:exp:DCOPF:exact_verification_hard}.}
    \label{tab:exp:DCOPF:exact_verification}
    \resizebox{\columnwidth}{!}{
    \scriptsize
    \begin{tabular}{lrrrr}
        \toprule
        System & \%$u$ &  Bilevel & Compact & \%Speedup  \\
        \midrule
        57 
         & 0 & 0.4 & \textbf{0.3} & 22.9 \\
         & 1 & \textbf{0.6} & 0.6 & -3.4 \\
         & 2 & 0.6 & \textbf{0.5} & 10.4 \\
         & 5 & 1.9 & \textbf{1.1} & 75.8 \\
         & 10 & \textbf{1.2} & 1.2 & -1.7 \\
         & 20 & 0.7 & \textbf{0.5} & 27.6 \\
        \midrule
        118 
         & 0 & 1.7 & \textbf{1.2} & 43.3 \\
         & 1 & 3.9 & \textbf{2.1} & 89.7 \\
         & 2 & 4.7 & \textbf{3.1} & 53.6 \\
         & 5 & 28.4 & \textbf{12.1} & 135.2 \\
         & 10 & 18.7 & \textbf{14.1} & 32.4 \\
         & 20 & 76.8 & \textbf{59.4} & 29.3 \\
        \midrule
        300 
         & 0 & 119.8 & \textbf{63.4} & 88.9 \\
         & 1 & 298.6 & \textbf{166.0} & 79.9 \\
         & 2 & 1302.7 & \textbf{420.8} & 209.5 \\
         & 5 & 17585.4 & \textbf{10507.9} & 67.4 \\
         \bottomrule
     \end{tabular}}
\end{table}

\begin{table}[!t]
    \centering
    \caption{Primal and dual objective value of \textcolor{blue}{open (unsolved)} instances. $\uparrow$ indicates the higher the better and $\downarrow$ indicates the lower the better}
    \label{tab:exp:DCOPF:exact_verification_hard}
    \resizebox{\columnwidth}{!}{
    \scriptsize
    \begin{tabular}{lrrrrrrr}
        \toprule
            &
            & \multicolumn{3}{c}{Primal (K\$) $\uparrow$}
            & \multicolumn{3}{c}{Dual (M\$) $\downarrow$} \\
        \cmidrule(lr){3-5}
        \cmidrule(lr){6-8}
        System &  \%$u$ &  Bilevel & Compact & \%PrimalGain & Bilevel & Compact & \%DualGain \\
        \midrule
        300 
         & 10 & 466.76 & 596.98 & 27.90 & 4.45 & 3.82 & 14.08 \\
         & 20 & 410.19 & 582.81 & 42.08 & 10.79 & 9.29 & 13.88 \\
        \midrule
        1,354 
         & 0 & 94.22 & 360.03 & 282.13 & 29.64 & 26.00 & 12.25 \\
         & 1 & 84.44 & 365.50 & 332.83 & 36.35 & 35.39 & 2.63 \\
         & 2 & 50.12 & 369.68 & 637.65 & 47.64 & 45.13 & 5.26 \\
         & 5 & 54.32 & 371.52 & 584.02 & 78.79 & 74.31 & 5.69 \\
         & 10 & 46.63 & 353.20 & 657.42 & 135.32 & 129.99 & 3.94 \\
         & 20 & 49.52 & 359.72 & 626.40 & 249.02 & 235.79 & 5.31 \\
         \bottomrule
     \end{tabular}}
\end{table}



\begin{figure*}
\centering
% \wc{Fix the captions}
\includegraphics[width=0.32\columnwidth]{figs/PrimalVal_vs_time/primal_obj_curve_300_ieee_0.05_hexagon_32.png}
\includegraphics[width=0.32\columnwidth]{figs/PrimalVal_vs_time/primal_obj_curve_300_ieee_0.06_hexagon_32.png}
\includegraphics[width=0.32\columnwidth]{figs/PrimalVal_vs_time/primal_obj_curve_300_ieee_0.07_hexagon_32.png}
\includegraphics[width=0.32\columnwidth]{figs/PrimalVal_vs_time/primal_obj_curve_300_ieee_0.1_hexagon_32.png}
\includegraphics[width=0.32\columnwidth]{figs/PrimalVal_vs_time/primal_obj_curve_300_ieee_0.15_hexagon_32.png}
\includegraphics[width=0.32\columnwidth]{figs/PrimalVal_vs_time/primal_obj_curve_300_ieee_0.25_hexagon_32.png} \\
\subfloat[0\%]{
\includegraphics[width=0.32\columnwidth]{figs/PrimalVal_vs_time/primal_obj_curve_1354_pegase_0.05_hexagon_32.png}}
\subfloat[1\%]{
\includegraphics[width=0.32\columnwidth]{figs/PrimalVal_vs_time/primal_obj_curve_1354_pegase_0.06_hexagon_32.png}}
\subfloat[2\%]{
\includegraphics[width=0.32\columnwidth]{figs/PrimalVal_vs_time/primal_obj_curve_1354_pegase_0.07_hexagon_32.png}}
\subfloat[5\%]{
\includegraphics[width=0.32\columnwidth]{figs/PrimalVal_vs_time/primal_obj_curve_1354_pegase_0.1_hexagon_32.png}}
\subfloat[10\%]{
\includegraphics[width=0.32\columnwidth]{figs/PrimalVal_vs_time/primal_obj_curve_1354_pegase_0.15_hexagon_32.png}}
\subfloat[20\%]{
\includegraphics[width=0.32\columnwidth]{figs/PrimalVal_vs_time/primal_obj_curve_1354_pegase_0.25_hexagon_32.png}}


    % \subfloat[]{
    %     \includegraphics[width=0.32\columnwidth]{figs/PrimalVal_vs_time/primal_obj_curve_300_ieee_0.05_hexagon_32.png}
    %     \label{fig:best_obj_val:DCOPF:300_ieee}
    % }
    % \subfloat[]{
    %     \includegraphics[width=0.32\columnwidth]{figs/PrimalVal_vs_time/primal_obj_curve_300_ieee_0.06_hexagon_32.png}
    %     \label{fig:best_obj_val:DCOPF:300_ieee}
    % }
    % \subfloat[]{
    %     \includegraphics[width=0.32\columnwidth]{figs/PrimalVal_vs_time/primal_obj_curve_300_ieee_0.07_hexagon_32.png}
    %     \label{fig:best_obj_val:DCOPF:300_ieee}
    % }
    % \subfloat[]{
    %     \includegraphics[width=0.32\columnwidth]{figs/PrimalVal_vs_time/primal_obj_curve_300_ieee_0.1_hexagon_32.png}
    %     \label{fig:best_obj_val:DCOPF:300_ieee}
    % }
    % \subfloat[ ]{
    %     \includegraphics[width=0.32\columnwidth]{figs/PrimalVal_vs_time/primal_obj_curve_300_ieee_0.15_hexagon_32.png}
    %     \label{fig:best_obj_val:DCOPF:300_ieee}
    % }
    % \subfloat[]{
    %     \includegraphics[width=0.32\columnwidth]{figs/PrimalVal_vs_time/primal_obj_curve_300_ieee_0.25_hexagon_32.png}
    %     \label{fig:best_obj_val:DCOPF:300_ieee}
    % } \\
    % \subfloat[1354 Pegase 0\% ]{
    %     \includegraphics[width=0.32\columnwidth]{figs/PrimalVal_vs_time/primal_obj_curve_1354_pegase_0.05_hexagon_32.png}
    %     \label{fig:best_obj_val:DCOPF:1354_pegase}
    % }
    % \subfloat[1354 Pegase 1\% ]{
    %     \includegraphics[width=0.32\columnwidth]{figs/PrimalVal_vs_time/primal_obj_curve_1354_pegase_0.06_hexagon_32.png}
    %     \label{fig:best_obj_val:DCOPF:1354_pegase}
    % }
    % \subfloat[1354 Pegase 2\% ]{
    %     \includegraphics[width=0.32\columnwidth]{figs/PrimalVal_vs_time/primal_obj_curve_1354_pegase_0.07_hexagon_32.png}
    %     \label{fig:best_obj_val:DCOPF:1354_pegase}
    % }
    % \subfloat[1354 Pegase 5\% ]{
    %     \includegraphics[width=0.32\columnwidth]{figs/PrimalVal_vs_time/primal_obj_curve_1354_pegase_0.1_hexagon_32.png}
    %     \label{fig:best_obj_val:DCOPF:1354_pegase}
    % }
    % \subfloat[1354 Pegase 10\% ]{
    %     \includegraphics[width=0.32\columnwidth]{figs/PrimalVal_vs_time/primal_obj_curve_1354_pegase_0.15_hexagon_32.png}
    %     \label{fig:best_obj_val:DCOPF:1354_pegase}
    % }
    % \subfloat[1354 Pegase 20\% ]{
    %     \includegraphics[width=0.32\columnwidth]{figs/PrimalVal_vs_time/primal_obj_curve_1354_pegase_0.25_hexagon_32.png}
    %     \label{fig:best_obj_val:DCOPF:1354_pegase}
    % }
    
    \caption{Evolution of primal objective value for compact and bilevel formulations overtime on 300 IEEE systems (top) and 1354 Pegase systems (bottom) with different sizes of input domains. Higher values indicate better outcomes.}
    \label{fig:primal_obj_val_along_time:DCOPF}
\end{figure*}

\iffalse{
\begin{figure*}
\centering
    
    \subfloat[300 IEEE 0\% ]{
        \includegraphics[width=0.32\columnwidth]{figs/DualVal_vs_time/dual_obj_curve_300_ieee_0.05_hexagon_32.png}
        \label{fig:dual_obj_val:DCOPF:300_ieee}
    }
    \subfloat[300 IEEE 1\% ]{
        \includegraphics[width=0.32\columnwidth]{figs/DualVal_vs_time/dual_obj_curve_300_ieee_0.06_hexagon_32.png}
        \label{fig:best_obj_val:DCOPF:300_ieee}
    }
    \subfloat[300 IEEE 2\% ]{
        \includegraphics[width=0.32\columnwidth]{figs/DualVal_vs_time/dual_obj_curve_300_ieee_0.07_hexagon_32.png}
        \label{fig:best_obj_val:DCOPF:300_ieee}
    }
    \subfloat[300 IEEE 5\% ]{
        \includegraphics[width=0.32\columnwidth]{figs/DualVal_vs_time/dual_obj_curve_300_ieee_0.1_hexagon_32.png}
        \label{fig:best_obj_val:DCOPF:300_ieee}
    }
    \subfloat[300 IEEE 10\% ]{
        \includegraphics[width=0.32\columnwidth]{figs/DualVal_vs_time/dual_obj_curve_300_ieee_0.15_hexagon_32.png}
        \label{fig:best_obj_val:DCOPF:300_ieee}
    }
    \subfloat[300 IEEE 20\% ]{
        \includegraphics[width=0.32\columnwidth]{figs/DualVal_vs_time/dual_obj_curve_300_ieee_0.25_hexagon_32.png}
        \label{fig:best_obj_val:DCOPF:300_ieee}
    } \\
    \subfloat[1354 Pegase 0\% ]{
        \includegraphics[width=0.32\columnwidth]{figs/DualVal_vs_time/dual_obj_curve_1354_pegase_0.05_hexagon_32.png}
        \label{fig:best_obj_val:DCOPF:1354_pegase}
    }
    \subfloat[1354 Pegase 1\% ]{
        \includegraphics[width=0.32\columnwidth]{figs/DualVal_vs_time/dual_obj_curve_1354_pegase_0.06_hexagon_32.png}
        \label{fig:best_obj_val:DCOPF:1354_pegase}
    }
    \subfloat[1354 Pegase 2\% ]{
        \includegraphics[width=0.32\columnwidth]{figs/DualVal_vs_time/dual_obj_curve_1354_pegase_0.07_hexagon_32.png}
        \label{fig:best_obj_val:DCOPF:1354_pegase}
    }
    \subfloat[1354 Pegase 5\% ]{
        \includegraphics[width=0.32\columnwidth]{figs/DualVal_vs_time/dual_obj_curve_1354_pegase_0.1_hexagon_32.png}
        \label{fig:best_obj_val:DCOPF:1354_pegase}
    }
    \subfloat[1354 Pegase 10\% ]{
        \includegraphics[width=0.32\columnwidth]{figs/DualVal_vs_time/dual_obj_curve_1354_pegase_0.15_hexagon_32.png}
        \label{fig:best_obj_val:DCOPF:1354_pegase}
    }
    \subfloat[1354 Pegase 20\% ]{
        \includegraphics[width=0.32\columnwidth]{figs/DualVal_vs_time/dual_obj_curve_1354_pegase_0.25_hexagon_32.png}
        \label{fig:best_obj_val:DCOPF:1354_pegase}
    }
    
    \caption{Evolution of Dual Values for Compact and Bilevel Formulations Over Time. Note: Lower values indicate better outcomes}
    \label{fig:dual_obj_val_along_time:DCOPF}
\end{figure*}
}\fi




\begin{table}[!t]
    \centering
    \caption{Comparisons of PGA-VFA and Compact formulation on final objective and solving time on large power systems.}
    \label{tab:exp:DCOPF:pga_vs_compact}
    \resizebox{\columnwidth}{!}{
    \scriptsize
    \begin{tabular}{lrrrrrrr}
        \toprule
            &
            & \multicolumn{2}{c}{PGA-VFA}
            & \multicolumn{2}{c}{Compact} \\
        \cmidrule(lr){3-4}
        \cmidrule(lr){5-6}
        System &  \%$u$ &  ObjVal (\$) & Time (s) &  ObjVal (\$) & Time (s) & $^{\dagger}$T2PGA (s) \\
        \midrule
        % 57 
        %  & 0 & 127.36 & 2.17 & 141.36 & 0.31 & 0.10 \\
        %  & 1 & 137.35 & 1.44 & 142.29 & 0.59 & 0.11 \\
        %  & 2 & 143.70 & 4.31 & 151.54 & 0.54 & 0.12 \\
        %  & 5 & 171.53 & 3.35 & 179.12 & 1.10 & 1.10 \\
        %  & 10 & 175.89 & 2.28 & 432.20 & 1.21 & 1.10 \\
        %  & 20 & 1527.72 & 5.59 & 3837.33 & 0.54 & 0.30 \\
        % \midrule
        % 118 
        %  & 0 & 752.29 & 1.43 & 6216.97 & 1.20 & 0.74 \\
        %  & 1 & 4615.37 & 6.96 & 7917.56 & 2.07 & 1.17 \\
        %  & 2 & 4615.37 & 7.61 & 9607.68 & 3.08 & 2.00 \\
        %  & 5 & 4615.37 & 4.44 & 14329.88 & 12.08 & 3.00 \\
        %  & 10 & 5448.69 & 6.26 & 68556.32 & 14.14 & 6.67 \\
        %  & 20 & 6048.77 & 9.04 & 69109.46 & 59.41 & 17.27 \\
        % \midrule
        300 
         & 0 & 544923.75 & 4.53 & 546038.13 & 63.41 & 52.06 \\
         & 1 & 562348.33 & 7.09 & 564263.39 & 166.01 & 114.79 \\
         & 2 & 572166.01 & 37.30 & 572464.17 & 420.83 & 307.40  \\
         & 5 & 572166.01 & 49.26 & 651163.59 & 10507.88 & 872.25 \\
         & 10 & 572166.01 & 41.41 & 596983.07 & t.o. & 2646.21  \\
         & 20 & 572166.01 & 17.86 & 582808.23 & t.o. & 2646.28 \\
        \midrule
        1,354 
         & 0 & 380673.60 & 67.26 & 360031.97 & t.o. & t.o.  \\
         & 1 & 399441.04 & 63.54 & 365497.51 & t.o. & t.o. \\
         & 2 & 403725.74 & 41.98 & 369678.23 & t.o. & t.o.\\
         & 5 & 403725.74 & 31.88 & 371524.52 & t.o. & t.o. \\
         & 10 & 571252.51 & 85.88 & 353196.16 & t.o. & t.o. \\
         & 20 & 571252.51 & 76.43 & 359722.30 & t.o. & t.o.  \\
         \bottomrule
    \end{tabular}}\\
    \footnotesize{$^{\dagger}$Time it took the compact formulation to reach the same primal objective as PGA.}
\end{table}

\begin{table}[!t]
    \centering
    \caption{Comparisons of PGA-VFA and Compact formulation with different warm starts.}
    % \mt{We should highlight that for hard instances (300 and 1354), Gurobi barely improves upon the PGA solution. In addition, for the 300-bus instances with 0\% -- 2\% noise, PGA appears to find a close-to-optimal solution.}
    \label{tab:pga_impact}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{lrrrr}
        \toprule
        System & \%$u$ & PGA-VFA & Compact (Nom) & Compact (PGA-VFA)\\
        \midrule
        % 57 
        %  & 0 & 127.36 & 141.36 & 141.36 \\
        %  & 1 & 137.35 & 142.29 & 142.29 \\
        %  & 2 & 143.70 & 151.54 & 151.54 \\
        %  & 5 & 171.53 & 179.12 & 179.12 \\
        %  & 10 & 175.89 & 432.20 & 432.21 \\
        %  & 20 & 1527.72 & 3837.33 & 3837.33 \\
        % \midrule
        % 118   
        %  & 0 & 752.29 & 6216.97 & 6216.97 \\
        %  & 1 & 4615.37 & 7917.56 & 7917.56 \\
        %  & 2 & 4615.37 & 9607.68 & 9607.68 \\
        %  & 5 & 4615.37 & 14329.88 & 14329.87 \\
        %  & 10 & 5448.69 & 68556.32 & 68556.32 \\
        %  & 20 & 6048.77 & 69109.46 & 69109.46 \\
        % \midrule
        300  
         & {\color{blue}0} & 544923.75 & 546038.13 & 546038.13 \\
         & {\color{blue}1} & 562348.32 & 564263.39 & 564263.44 \\
         & {\color{blue}2} & 572166.01 & 572464.17 & 572464.17 \\
         & {\color{blue}5} & 572166.01 & 651163.59 & 651163.38 \\
         & 10 & 572166.01 & 596983.07 & 596983.90 \\
         & 20 & 572166.01 & 582808.23 & 582808.47 \\
        \midrule
        1,354 
         & 0 & 380673.60 & 360031.97 & 380757.88 \\
         & 1 & 399441.04 & 365497.51 & 399579.63 \\
         & 2 & 403725.74 & 369678.23 & 406165.38 \\
         & 5 & 403725.74 & 371524.52 & 406164.74 \\
         & 10 & 571252.51 & 353196.16 & 571715.99 \\
         & 20 & 571252.51 & 359722.30 & 578732.15 \\
         \bottomrule
    \end{tabular}
    }
    % \mt{\textbf{Take-away from this table}: passing PGA warm-start to Gurobi always yields better primal solutions that passing nominal warm-start. Important note: the bilevel formulation will sometimes reject the warm-start because Gurobi cannot complete the (bilevel-feasible) solution within its work limits; this never happens with our compact formulation.}
\end{table}

\iffalse{
\begin{table*}[!t]
    \centering
    \caption{Computing time and final primal and dual values. The t.o. stands for the solving hits a time limit of 6 hours. The instances that are solved to optimal are marked in  {\color{blue}{blue}}, where the Primal value is equal to the Dual value. Higher Primal value and lower Dual value indicate better performance.}
    \label{tab:exp:DCOPF:computing_times_nominal}
    % \mt{Did these experiments use any bound tightening before solving the MIP? If so, which one?}
    % \wc{All instances are solved using OBBT for bound tightening and pgd for warm start.}
    % \resizebox{\columnwidth}{!}{
    \resizebox{\linewidth}{!}{
    \scriptsize
    \begin{tabular}{lrrrrrrrrrr}
        \toprule
            &
            & \multicolumn{3}{c}{Bilevel}
            & \multicolumn{3}{c}{Compact}\\
        \cmidrule(lr){3-5}
        \cmidrule(lr){6-8}
        System & \%$u$ &  Time (s) & Primal (\$) $\uparrow$  & Dual (\$) $\downarrow$ &  Time (s) & Primal (\$) $\uparrow$  & Dual (\$) $\downarrow$ & \%Speedup & \%Primal & \%Dual  \\
        \midrule
         \color{blue}{57}
         & \color{blue}{0} & 0.4 & 141.4 & 141.4 & 0.3 & 141.4 & 141.4 & 122.9 & - & - \\
         &  \color{blue}{1} & 0.6 & 142.3 & 142.3 & 0.6 & 142.3 & 142.3 & 96.6 & - & - \\
         &  \color{blue}{2} & 0.6 & 151.5 & 151.5 & 0.5 & 151.5 & 151.5 & 110.4 & - & - \\
         &  \color{blue}{5} & 1.9 & 179.1 & 179.1 & 1.1 & 179.1 & 179.1 & 175.8 & - & - \\
         &  \color{blue}{10} & 1.2 & 432.2 & 432.2 & 1.2 & 432.2 & 432.2 & 98.3 & - & - \\
         &  \color{blue}{20} & 0.7 & 3837.3 & 3837.3 & 0.5 & 3837.3 & 3837.3 & 127.6 & - & - \\
        \midrule
         \color{blue}{118} 
         &  \color{blue}{0} & 1.7 & 6217.0 & 6217.0 & 1.2 & 6217.0 & 6217.0 & 143.3 & - & - \\
         &  \color{blue}{1} & 3.9 & 7917.6 & 7917.6 & 2.1 & 7917.6 & 7917.6 & 189.7 & - & - \\
         &  \color{blue}{2} & 4.7 & 9607.7 & 9607.7 & 3.1 & 9607.7 & 9607.7 & 153.6 & - & - \\
         &  \color{blue}{5} & 28.4 & 14329.9 & 14329.9 & 12.1 & 14329.9 & 14329.9 & 235.2 & - & - \\
         &  \color{blue}{10} & 18.7 & 68556.3 & 68556.3 & 14.1 & 68556.3 & 68556.3 & 132.4 & - & - \\
         &  \color{blue}{20} & 76.8 & 69109.5 & 69109.5 & 59.4 & 69109.5 & 69109.5 & 129.3 & - & - \\
        \midrule
        300
         &  \color{blue}{0} & 119.8 & 546038.1 & 546038.2 & 63.4 & 546038.1 & 546038.2 & 188.9 & - & - \\
         &  \color{blue}{1} & 298.6 & 564263.4 & 564263.4 & 166.0 & 564263.4 & 564263.4 & 179.9 & - & - \\
         &  \color{blue}{2} & 1302.7 & 572464.2 & 572464.2 & 420.8 & 572464.2 & 572464.2 & 309.5 & - & - \\
         &  \color{blue}{5} & 17585.4 & 651163.8 & 651163.6 & 10507.9 & 651163.6 & 651163.6 & 167.4 & - & - \\
         & 10 & t.o. & 466762.9 & 4450478.5 & t.o. & 596983.1 & 3823954.9 & - & 27.9 & 14.1 \\
         & 20 & t.o. & 410189.7 & 10787349.0 & t.o. & 582808.2 & 9289811.0 & - & 42.1 & 13.9 \\
        \midrule
        1,354 
         & 0 & t.o. & 94216.8 & 29636173.4 & t.o. & 360032.0 & 26004295.5 & - & 282.1 & 12.3 \\
         & 1 & t.o. & 84443.6 & 36346463.2 & t.o. & 365497.5 & 35391272.9 & - & 332.8 & 2.6 \\
         & 2 & t.o. & 50115.7 & 47635747.5 & t.o. & 369678.2 & 45131282.0 & - & 637.6 & 5.3 \\
         & 5 & t.o. & 54315.2 & 78790475.6 & t.o. & 371524.5 & 74308992.4 & - & 584.0 & 5.7 \\
         & 10 & t.o. & 46631.5 & 135324003.0 & t.o. & 353196.2 & 129986251.0 & - & 657.4 & 3.9 \\
         & 20 & t.o. & 49521.1 & 249022961.0 & t.o. & 359722.3 & 235794640.0 & - & 626.4 & 5.3 \\
         \bottomrule
     \end{tabular}}
\end{table*}


\begin{table}[!t]
    \centering
    \caption{Computing time and final gap}
    \label{tab:exp:DCOPF:computing_times_nominal}
    % \mt{Did these experiments use any bound tightening before solving the MIP? If so, which one?}
    % \wc{All instances are solved using OBBT for bound tightening and pgd for warm start.}
    \resizebox{\columnwidth}{!}{
    \scriptsize
    \begin{tabular}{lrrrrrrr}
        \toprule
            &
            & \multicolumn{2}{c}{Bilevel}
            & \multicolumn{2}{c}{Compact}\\
        \cmidrule(lr){3-4}
        \cmidrule(lr){5-6}
        System & \%$u$ &  Time (s) & \%Gap &  Time (s) & \%Gap & \%Speedup & \%GapDrop  \\
        \midrule
        57 
         & 0 & 0.4 & 0.0 & 0.3 & 0.0 & 18.6 & - \\
         & 1 & 0.6 & 0.0 & 0.6 & 0.0 & -3.5 & - \\
         & 2 & 0.6 & 0.0 & 0.5 & 0.0 & 9.4 & - \\
         & 5 & 1.9 & 0.0 & 1.1 & 0.0 & 43.1 & - \\
         & 10 & 1.2 & 0.0 & 1.2 & 0.0 & -1.7 & - \\
         & 20 & 0.7 & 0.0 & 0.5 & 0.0 & 21.7 & - \\
        \midrule
        118 
         & 0 & 1.7 & 0.0 & 1.2 & 0.0 & 30.2 & - \\
         & 1 & 3.9 & 0.0 & 2.1 & 0.0 & 47.3 & - \\
         & 2 & 4.7 & 0.0 & 3.1 & 0.0 & 34.9 & - \\
         & 5 & 28.4 & 0.0 & 12.1 & 0.0 & 57.5 & - \\
         & 10 & 18.7 & 0.0 & 14.1 & 0.0 & 24.5 & - \\
         & 20 & 76.8 & 0.0 & 59.4 & 0.0 & 22.7 & - \\
        \midrule
        300
         & 0 & 119.8 & 0.0 & 63.4 & 0.0 & 47.1 & - \\
         & 1 & 298.6 & 0.0 & 166.0 & 0.0 & 44.4 & - \\
         & 2 & 1302.7 & 0.0 & 420.8 & 0.0 & 67.7 & - \\
         & 5 & 17585.4 & 0.0 & 10507.9 & 0.0 & 40.2 & - \\
         & 10 & t.o. & 802.3 & t.o. & 530.7 & - & 33.8 \\
         & 20 & t.o. & 3054.0 & t.o. & 1493.2 & - & 51.1 \\
        \midrule
        1,354 
         & 0 & t.o. & 31340.3 & t.o. & 7122.0 & - & 77.3 \\
         & 1 & t.o. & 42924.6 & t.o. & 9582.9 & - & 77.7 \\
         & 2 & t.o. & 94933.6 & t.o. & 12108.0 & - & 87.2 \\
         & 5 & t.o. & 144957.5 & t.o. & 19901.0 & - & 86.3 \\
         & 10 & t.o. & 290089.9 & t.o. & 36702.7 & - & 87.3 \\
         & 20 & t.o. & 502745.4 & t.o. & 65448.9 & - & 87.0 \\
         \bottomrule
     \end{tabular}}
\end{table}


\begin{table}[!t]
    \centering
    \caption{Relative Optimality Gap achieved by each method. Each number is the geometric mean over 5 random seeds.}
    \mt{We should highlight that for hard instances (300 and 1354), Gurobi barely improves upon the PGA solution. In addition, for the 300-bus instances with 0\% -- 2\% noise, PGA appears to find a close-to-optimal solution.}
    \label{tab:primal_performance}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{lrrrrrrr}
        \toprule
            &
            & \multicolumn{2}{c}{Heuristic}
            & \multicolumn{2}{c}{Compact}
            & \multicolumn{2}{c}{Bilevel}\\
        \cmidrule(lr){3-4}
        \cmidrule(lr){5-6}
        \cmidrule(lr){7-8}
        System & $\mu$ (\%) &  Nom. & PGA & Nom & PGA & Nom & PGA\\
        \midrule
        57 
         & 0 & 213.55 & 10.99 & 0.00 & 0.00 & 0.00 & 0.00 \\
         & 1 & 215.63 & 3.59 & 0.00 & 0.00 & 0.00 & 0.00 \\
         & 2 & 236.13 & 5.45 & 0.00 & 0.00 & 0.00 & 0.00 \\
         & 5 & 297.33 & 4.42 & 0.00 & 0.00 & 0.00 & 0.00 \\
         & 10 & 858.71 & 145.73 & 0.00 & 0.00 & 0.00 & 0.00 \\
         & 20 & 8411.79 & 151.18 & 0.00 & 0.00 & 0.00 & 0.00 \\
        \midrule
        118   
         & 0 & 3317.46 & 726.41 & 0.00 & 0.00 & 0.00 & 0.00 \\
         & 1 & 4252.27 & 71.55 & 0.00 & 0.00 & 0.00 & 0.00 \\
         & 2 & 5181.33 & 108.17 & 0.00 & 0.00 & 0.00 & 0.00 \\
         & 5 & 7777.12 & 210.48 & 0.00 & 0.00 & 0.00 & 0.00 \\
         & 10 & 37585.33 & 1158.22 & 0.00 & 0.00 & 0.00 & 0.00 \\
         & 20 & 37889.43 & 1042.54 & 0.00 & 0.00 & 0.00 & 0.00 \\
        \midrule
        300  
         & 0 & 12980.84 & 0.20 & 0.00 & 0.00 & 0.00 & 0.00 \\
         & 1 & 13417.43 & 0.34 & 0.00 & 0.00 & 0.00 & 0.00 \\
         & 2 & 13613.89 & 0.05 & 0.00 & 0.00 & 0.00 & 0.00 \\
         & 5 & 15499.21 & 13.81 & 0.00 & 0.00 & 0.00 & 0.00 \\
         & 10 & 14201.28 & 4.34 & 0.00 & 0.00 & 27.90 & 2.43 \\
         & 20 & 13861.69 & 1.86 & 0.00 & 0.00 & 42.08 & 0.00 \\
        \midrule
        1,354 
         & 0 & 5098.80 & 0.02 & 5.76 & 0.00 & 304.13 & 0.00 \\
         & 1 & 5355.79 & 0.03 & 9.32 & 0.00 & 373.19 & 0.00 \\
         & 2 & 5445.71 & 0.60 & 9.87 & 0.00 & 710.45 & 0.00 \\
         & 5 & 5445.70 & 0.60 & 9.32 & 0.00 & 647.79 & 0.00 \\
         & 10 & 7706.10 & 0.08 & 61.87 & 0.00 & 1126.03 & 0.00 \\
         & 20 & 7801.90 & 1.31 & 60.88 & 0.00 & 1068.66 & 0.03\\
         \bottomrule
    \end{tabular}
    }
    \mt{\textbf{Take-away from this table}: passing PGA warm-start to Gurobi always yields better primal solutions that passing nominal warm-start. Important note: the bilevel formulation will sometimes reject the warm-start because Gurobi cannot complete the (bilevel-feasible) solution within its work limits; this never happens with our compact formulation.}
\end{table}


\begin{table}[!t]
    \centering
    \caption{Relative Optimality Gap achieved by each method. Each number is the geometric mean over 5 random seeds.}
    \wc{Need a table to show the performance of PGA}
    \mt{We should highlight that for hard instances (300 and 1354), Gurobi barely improves upon the PGA solution. In addition, for the 300-bus instances with 0\% -- 2\% noise, PGA appears to find a close-to-optimal solution.}
    \label{tab:primal_performance}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{lrrrrrrr}
        \toprule
            &
            & \multicolumn{2}{c}{Heuristic}
            & \multicolumn{2}{c}{Compact}
            & \multicolumn{2}{c}{Bilevel}\\
        \cmidrule(lr){3-4}
        \cmidrule(lr){5-6}
        \cmidrule(lr){7-8}
        System & $\alpha$ (\%) &  Nom. & PGA & Nom & PGA & Nom & PGA\\
        \midrule
        57 
         & 0 & 213.55 & 10.99 & 0.00 & 0.00 & 0.00 & 0.00 \\
         & 1 & 215.63 & 3.59 & 0.00 & 0.00 & 0.00 & 0.00 \\
         & 2 & 236.13 & 5.45 & 0.00 & 0.00 & 0.00 & 0.00 \\
         & 5 & 297.33 & 4.42 & 0.00 & 0.00 & 0.00 & 0.00 \\
         & 10 & 858.71 & 145.73 & 0.00 & 0.00 & 0.00 & 0.00 \\
         & 20 & 8411.79 & 151.18 & 0.00 & 0.00 & 0.00 & 0.00 \\
        \midrule
        118   
         & 0 & 3317.46 & 726.41 & 0.00 & 0.00 & 0.00 & 0.00 \\
         & 1 & 4252.27 & 71.55 & 0.00 & 0.00 & 0.00 & 0.00 \\
         & 2 & 5181.33 & 108.17 & 0.00 & 0.00 & 0.00 & 0.00 \\
         & 5 & 7777.12 & 210.48 & 0.00 & 0.00 & 0.00 & 0.00 \\
         & 10 & 37585.33 & 1158.22 & 0.00 & 0.00 & 0.00 & 0.00 \\
         & 20 & 37889.43 & 1042.54 & 0.00 & 0.00 & 0.00 & 0.00 \\
        \midrule
        300  
         & 0 & 12980.84 & 0.20 & 0.00 & 0.00 & 0.00 & 0.00 \\
         & 1 & 13417.43 & 0.34 & 0.00 & 0.00 & 0.00 & 0.00 \\
         & 2 & 13613.89 & 0.05 & 0.00 & 0.00 & 0.00 & 0.00 \\
         & 5 & 15499.21 & 13.81 & 0.00 & 0.00 & 0.00 & 0.00 \\
         & 10 & 14201.28 & 4.34 & 0.00 & 0.00 & 27.90 & 2.43 \\
         & 20 & 13861.69 & 1.86 & 0.00 & 0.00 & 42.08 & 0.00 \\
        \midrule
        1,354 
         & 0 & 5098.80 & 0.02 & 5.76 & 0.00 & 304.13 & 0.00 \\
         & 1 & 5355.79 & 0.03 & 9.32 & 0.00 & 373.19 & 0.00 \\
         & 2 & 5445.71 & 0.60 & 9.87 & 0.00 & 710.45 & 0.00 \\
         & 5 & 5445.70 & 0.60 & 9.32 & 0.00 & 647.79 & 0.00 \\
         & 10 & 7706.10 & 0.08 & 61.87 & 0.00 & 1126.03 & 0.00 \\
         & 20 & 7801.90 & 1.31 & 60.88 & 0.00 & 1068.66 & 0.03\\
         \bottomrule
    \end{tabular}
    }
    \mt{\textbf{Take-away from this table}: passing PGA warm-start to Gurobi always yields better primal solutions that passing nominal warm-start. Important note: the bilevel formulation will sometimes reject the warm-start because Gurobi cannot complete the (bilevel-feasible) solution within its work limits; this never happens with our compact formulation.}
\end{table}

\begin{table}[!t]
    \centering
    \caption{Computing time and final gap with PGA Warm Start}
    \label{tab:exp:DCOPF:computing_times}
    % \mt{Did these experiments use any bound tightening before solving the MIP? If so, which one?}
    % \wc{All instances are solved using OBBT for bound tightening and pgd for warm start.}
    % \resizebox{\columnwidth}{!}{
    \scriptsize
    \begin{tabular}{lrrrrrr}
        \toprule
            &
            & \multicolumn{2}{c}{Compact}
            & \multicolumn{2}{c}{Bilevel}\\
        \cmidrule(lr){3-4}
        \cmidrule(lr){5-6}
        System & $\alpha$ (\%) &  Time (s) & \%Gap &  Time (s) & \%Gap & \%Speedup  \\
        \midrule
        57 
         & 0 & 0.33 & 0 & 0.36 & 0  & 7.32 \\
         & 1 & 0.56 & 0 & 0.57 & 0  & 1.91 \\
         & 2 & 0.55 & 0 & 0.55 & 0  & 1.50 \\
         & 5 & 1.08 & 0 & 1.18 & 0  & 8.61 \\
         & 10 & 1.21 & 0 & 1.40 & 0 & 13.72 \\
         & 20 & 0.39 & 0 & 0.49 & 0 & 18.93 \\
        \midrule
        118 
         & 0 & 1.40 & 0 & 1.94 & 0    & 28.08 \\
         & 1 & 2.11 & 0 & 3.35 & 0    & 36.85 \\
         & 2 & 2.68 & 0 & 4.06 & 0    & 34.09 \\
         & 5 & 10.90 & 0 & 16.30 & 0  & 33.15 \\
         & 10 & 15.91 & 0 & 22.71 & 0 & 29.93 \\
         & 20 & 61.14 & 0 & 69.83 & 0 & 12.44 \\
        \midrule
        300 
         & 0 & 62.80 & 0 & 137.64 & 0      & 54.38 \\
         & 1 & 128.72 & 0 & 244.36 & 0     & 47.33 \\
         & 2 & 395.03 & 0 & 500.31 & 0     & 21.04 \\
         & 5 & 11265.36 & 0 & 11844.66 & 0 & 4.89 \\
         & 10 & t.o. & 532 & t.o. & 691    & - \\
         & 20 & t.o. & 2425 & t.o. & 2664  & - \\
        \midrule
        1,354 
         & 0 & t.o. & 7146 & t.o. & 6677    & - \\
         & 1 & t.o. & 8472 & t.o. & 9644    & - \\
         & 2 & t.o. & 10664 & t.o. & 11481  & - \\
         & 5 & t.o. & 18365 & t.o. & 18366  & - \\
         & 10 & t.o. & 21562 & t.o. & 23583 & - \\
         & 20 & t.o. & 40480 & t.o. & 42181 & - \\
         \bottomrule
    \end{tabular}
\end{table}

\begin{table}[!t]
    \centering
    \caption{Best primal objective value achieved by each method. Each number is the geometric mean over 5 random seeds.}
    % \wc{New results updated 01/20}
    \mt{We should highlight that for hard instances (300 and 1354), Gurobi barely improves upon the PGA solution. In addition, for the 300-bus instances with 0\% -- 2\% noise, PGA appears to find a close-to-optimal solution.}
    \label{tab:primal_performance}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{lrrrrrrr}
        \toprule
            &
            & \multicolumn{2}{c}{Heuristic}
            & \multicolumn{2}{c}{Compact}
            & \multicolumn{2}{c}{Bilevel}\\
        \cmidrule(lr){3-4}
        \cmidrule(lr){5-6}
        \cmidrule(lr){7-8}
        System & Noise (\%) &  Nom. & PGA & Nom & PGA & Nom & PGA\\
        \midrule
        57 
        & 0 & 45.08 & 127.36 & 141.36 & 141.36 & 141.36 & 141.36 \\
         & 1 & 45.08 & 137.35 & 142.29 & 142.29 & 142.29 & 142.29 \\
         & 2 & 45.08 & 143.70 & 151.54 & 151.54 & 151.54 & 151.54 \\
         & 5 & 45.08 & 171.53 & 179.12 & 179.12 & 179.12 & 179.12 \\
         & 10 & 45.08 & 175.89 & 432.20 & 432.21 & 432.20 & 432.21 \\
         & 20 & 45.08 & 1527.72 & 3837.33 & 3837.33 & 3837.33 & 3837.33 \\
        \midrule
        118   
        & 0 & 181.92 & 752.29 & 6216.97 & 6216.97 & 6216.97 & 6216.97 \\
         & 1 & 181.92 & 4615.37 & 7917.56 & 7917.56 & 7917.56 & 7917.56 \\
         & 2 & 181.92 & 4615.37 & 9607.68 & 9607.68 & 9607.68 & 9607.68 \\
         & 5 & 181.92 & 4615.37 & 14329.88 & 14329.87 & 14329.86 & 14329.86 \\
         & 10 & 181.92 & 5448.69 & 68556.32 & 68556.32 & 68556.32 & 68556.32 \\
         & 20 & 181.92 & 6048.77 & 69109.46 & 69109.46 & 69109.46 & 69109.51 \\
        \midrule
        300  
         & 0 & 4174.34 & 544923.75 & 546038.13 & 546038.13 & 546038.15 & 546038.55 \\
         & 1 & 4174.34 & 562348.32 & 564263.39 & 564263.44 & 564263.38 & 564263.40 \\
         & 2 & 4174.34 & 572166.01 & 572464.17 & 572464.17 & 572464.17 & 572460.26 \\
         & 5 & 4174.34 & 572166.01 & 651163.59 & 651163.38 & 651163.82 & 651163.54 \\
         & 10 & 4174.34 & 572166.01 & 596983.07 & 596983.90 & 466762.90 & 582808.43 \\
         & 20 & 4174.34 & 572166.01 & 582808.23 & 582808.47 & 410189.68 & 582808.47 \\
        \midrule
        1354 
         & 0 & 7323.96 & 380673.60 & 360031.97 & 380757.88 & 94216.80 & 380757.91 \\
         & 1 & 7323.96 & 399441.04 & 365497.51 & 399579.63 & 84443.61 & 399579.59 \\
         & 2 & 7323.96 & 403725.74 & 369678.23 & 406165.38 & 50115.73 & 406164.66 \\
         & 5 & 7323.96 & 403725.74 & 371524.52 & 406164.74 & 54315.20 & 406164.55 \\
         & 10 & 7323.96 & 571252.51 & 353196.16 & 571715.99 & 46631.55 & 571715.59 \\
         & 20 & 7323.96 & 571252.51 & 359722.30 & 578732.15 & 49521.07 & 578550.40 \\
         \bottomrule
    \end{tabular}
    }
    \mt{\textbf{Take-away from this table}: passing PGA warm-start to Gurobi always yields better primal solutions that passing nominal warm-start. Important note: the bilevel formulation will sometimes reject the warm-start because Gurobi cannot complete the (bilevel-feasible) solution within its work limits; this never happens with our compact formulation.}
\end{table}
}\fi

\paragraph{Effectiveness of Compact Formulation}
Table \ref{tab:exp:DCOPF:exact_verification} reports the solving time and optimality of the Compact formulation and Bilevel formulation on instances that can be solved to optimality.
The \%Speedup computes
\(\frac{t_{\text{Bilevel}} - t_{\text{Compact}}}{t_{\text{Compact}}} \times 100\%.\)
The Compact formulation consistently outperforms the Bilevel formulation except in two small instances where both formulations could be solved within 2 seconds.
Notably, the Compact formulation tends to achieve higher \%Speedup on larger systems, with up to 209.5\% on 300 bus systems with 2\% input perturbation.
Table \ref{tab:exp:DCOPF:exact_verification_hard} reports the performance of two formulations on open instances, where none of the formulations can solve the instances to optimality within 6 hours, primarily due to the weak linear relaxation.
In this case, the comparison focuses on the final primal and dual objective. The \%PrimalGain and \%DualGain report the performance improvement on the primal and dual side, respectively:
\(\frac{\text{Dual}_{\text{Bilevel}} - \text{Dual}_{\text{Compact}}}{\text{Dual}_{\text{Bilevel}}} \times 100\%\) and 
\(\frac{\text{Primal}_{\text{Compact}} - \text{Primal}_{\text{Bilevel}}}{\text{Dual}_{\text{Bilevel}}} \times 100\%.\)
As reported in Table \ref{tab:exp:DCOPF:exact_verification_hard}, the Compact formulation can find significantly better primal solutions than the Bilevel formulation especially when instances get harder (as suggested by a sharp increase of \%Primal). This is further supported in Figure \ref{fig:primal_obj_val_along_time:DCOPF}, where the Compact formulation consistently convergence faster along solving time.
On the dual side, the Compact formulation is slightly better than the Bilevel counterparts.
Since the Compact formulation systematically outperforms the Bilevel formulation, the later experiments focus on the Compact formulation.

\paragraph{Effectiveness of PGA-VFA}
\wc{define the nominal load somewhere}
Table \ref{tab:exp:DCOPF:pga_vs_compact} focuses on the performance of the proposed PGA-VFA and Compact formulation on large power systems (300 bus and 1364 bus).
The performances on small systems are deferred to Appendix \ref{appendix:dcopf:more_results} since Compact formulation solves those instances within 60 seconds. 
PGA-VFA is particularly good at finding high-quality primal solutions. It finds near-optimal solutions on 300 systems with orders of magnitude faster than the Compact formulation with a nominal warm start.
Notably, the compact model with a nominal warm start cannot find the same quality of primal solutions as PGA-VFA on 1354 systems within 6 hours.

Finally, Table \ref{tab:pga_impact} reports the impact of warm starting solution of PGA-VFA to Compact formulation.
First, the Compact models with PGA-VFA solutions as warm start always outperform their counterparts with nominal warm starts.
Second, the Compact model can barely improve on the PGA-VFA solutions because PGA-VFA achieves near-optimal solutions (for the instance marked in {\color{blue}blue}) or Gurobi struggles finding better primal solutions within 6 hours.



% \begin{figure}
% \wc{Compact formulation has better convergence along time than the Bilevel formulation}
% \centering
    
%     % \subfloat[300 IEEE 0\% ]{
%     %     \includegraphics[width=0.33\columnwidth]{figs/BestObjVal_vs_time/pgd_obj_curve_300_ieee_0.05_hexagon_32.png}
%     %     \label{fig:best_obj_val:DCOPF:300_ieee}
%     % }
%     % \subfloat[300 IEEE 1\% ]{
%     %     \includegraphics[width=0.33\columnwidth]{figs/BestObjVal_vs_time/pgd_obj_curve_300_ieee_0.06_hexagon_32.png}
%     %     \label{fig:best_obj_val:DCOPF:300_ieee}
%     % }
%     \subfloat[300 IEEE 2\% ]{
%         \includegraphics[width=0.32\columnwidth]{figs/BestObjVal_vs_time/pgd_obj_curve_300_ieee_0.07_hexagon_32.png}
%         \label{fig:best_obj_val:DCOPF:300_ieee}
%     }
%     \subfloat[300 IEEE 5\% ]{
%         \includegraphics[width=0.32\columnwidth]{figs/BestObjVal_vs_time/pgd_obj_curve_300_ieee_0.1_hexagon_32.png}
%         \label{fig:best_obj_val:DCOPF:300_ieee}
%     }
%     \subfloat[300 IEEE 10\% ]{
%         \includegraphics[width=0.32\columnwidth]{figs/BestObjVal_vs_time/pgd_obj_curve_300_ieee_0.15_hexagon_32.png}
%         \label{fig:best_obj_val:DCOPF:300_ieee}
%     }
%     % \subfloat[300 IEEE 20\% ]{
%     %     \includegraphics[width=0.33\columnwidth]{figs/BestObjVal_vs_time/pgd_obj_curve_300_ieee_0.25_hexagon_32.png}
%     %     \label{fig:best_obj_val:DCOPF:300_ieee}
%     % }
%     % \subfloat[1354 Pegase 0\% ]{
%     %     \includegraphics[width=0.33\columnwidth]{figs/BestObjVal_vs_time/pgd_obj_curve_1354_pegase_0.05_hexagon_32.png}
%     %     \label{fig:best_obj_val:DCOPF:1354_pegase}
%     % }
%     % \subfloat[1354 Pegase 1\% ]{
%     %     \includegraphics[width=0.33\columnwidth]{figs/BestObjVal_vs_time/pgd_obj_curve_1354_pegase_0.06_hexagon_32.png}
%     %     \label{fig:best_obj_val:DCOPF:1354_pegase}
%     % }
%     % \subfloat[1354 Pegase 2\% ]{
%     %     \includegraphics[width=0.33\columnwidth]{figs/BestObjVal_vs_time/pgd_obj_curve_1354_pegase_0.07_hexagon_32.png}
%     %     \label{fig:best_obj_val:DCOPF:1354_pegase}
%     % }
%     % \subfloat[1354 Pegase 5\% ]{
%     %     \includegraphics[width=0.33\columnwidth]{figs/BestObjVal_vs_time/pgd_obj_curve_1354_pegase_0.1_hexagon_32.png}
%     %     \label{fig:best_obj_val:DCOPF:1354_pegase}
%     % }
%     % \subfloat[1354 Pegase 10\% ]{
%     %     \includegraphics[width=0.33\columnwidth]{figs/BestObjVal_vs_time/pgd_obj_curve_1354_pegase_0.15_hexagon_32.png}
%     %     \label{fig:best_obj_val:DCOPF:1354_pegase}
%     % }
%     % \subfloat[1354 Pegase 20\% ]{
%     %     \includegraphics[width=0.33\columnwidth]{figs/BestObjVal_vs_time/pgd_obj_curve_1354_pegase_0.25_hexagon_32.png}
%     %     \label{fig:best_obj_val:DCOPF:1354_pegase}
%     % }
    
%     \mt{I would only keep 300+2\% and 300+10\% to illustrate that 1) Gurobi+bilevel may reject the warm-start, and 2) compact is the only one that ever manages to outperform PGA. All other instances are either "solved," or no significant difference. We could keep 300+5\% to indicate that 3) sometimes we can improve on PGA and 4) smaller input domain can yield better primal solutions faster. This last observation could be related to the input domain partitioning strategy for PGA.}
%     \caption{Best objective value along time}
%     \label{fig:best_obj_val_along_time:DCOPF}
% \end{figure}

\iffalse{
\begin{figure*}
\wc{Compact formulation has better convergence along time than the Bilevel formulation}
    \centering
    \subfloat[118 IEEE 0\%]{
        \includegraphics[width=0.33\columnwidth]{figs/BestObjVal_vs_time/pgd_obj_curve_118_ieee_0.05_hexagon_32.png}
        \label{fig:best_obj_val:DCOPF:118_ieee}
    }
    \subfloat[118 IEEE 1\%]{
        \includegraphics[width=0.33\columnwidth]{figs/BestObjVal_vs_time/pgd_obj_curve_118_ieee_0.06_hexagon_32.png}
        \label{fig:best_obj_val:DCOPF:118_ieee}
    }
    \subfloat[118 IEEE 2\% ]{
        \includegraphics[width=0.33\columnwidth]{figs/BestObjVal_vs_time/pgd_obj_curve_118_ieee_0.07_hexagon_32.png}
        \label{fig:best_obj_val:DCOPF:118_ieee}
    }
    \subfloat[118 IEEE 5\% ]{
        \includegraphics[width=0.33\columnwidth]{figs/BestObjVal_vs_time/pgd_obj_curve_118_ieee_0.1_hexagon_32.png}
        \label{fig:best_obj_val:DCOPF:118_ieee}
    }
    \subfloat[118 IEEE 10\% ]{
        \includegraphics[width=0.33\columnwidth]{figs/BestObjVal_vs_time/pgd_obj_curve_118_ieee_0.15_hexagon_32.png}
        \label{fig:best_obj_val:DCOPF:118_ieee}
    }
    \subfloat[118 IEEE 20\% ]{
        \includegraphics[width=0.33\columnwidth]{figs/BestObjVal_vs_time/pgd_obj_curve_118_ieee_0.25_hexagon_32.png}
        \label{fig:best_obj_val:DCOPF:118_ieee}
    }\\
    
    \subfloat[300 IEEE 0\% ]{
        \includegraphics[width=0.33\columnwidth]{figs/BestObjVal_vs_time/pgd_obj_curve_300_ieee_0.05_hexagon_32.png}
        \label{fig:best_obj_val:DCOPF:300_ieee}
    }
    \subfloat[300 IEEE 1\% ]{
        \includegraphics[width=0.33\columnwidth]{figs/BestObjVal_vs_time/pgd_obj_curve_300_ieee_0.06_hexagon_32.png}
        \label{fig:best_obj_val:DCOPF:300_ieee}
    }
    \subfloat[300 IEEE 2\% ]{
        \includegraphics[width=0.33\columnwidth]{figs/BestObjVal_vs_time/pgd_obj_curve_300_ieee_0.07_hexagon_32.png}
        \label{fig:best_obj_val:DCOPF:300_ieee}
    }
    \subfloat[300 IEEE 5\% ]{
        \includegraphics[width=0.33\columnwidth]{figs/BestObjVal_vs_time/pgd_obj_curve_300_ieee_0.1_hexagon_32.png}
        \label{fig:best_obj_val:DCOPF:300_ieee}
    }
    \subfloat[300 IEEE 10\% ]{
        \includegraphics[width=0.33\columnwidth]{figs/BestObjVal_vs_time/pgd_obj_curve_300_ieee_0.15_hexagon_32.png}
        \label{fig:best_obj_val:DCOPF:300_ieee}
    }
    \subfloat[300 IEEE 20\% ]{
        \includegraphics[width=0.33\columnwidth]{figs/BestObjVal_vs_time/pgd_obj_curve_300_ieee_0.25_hexagon_32.png}
        \label{fig:best_obj_val:DCOPF:300_ieee}
    }\\

    \subfloat[1354 Pegase 0\% ]{
        \includegraphics[width=0.33\columnwidth]{figs/BestObjVal_vs_time/pgd_obj_curve_1354_pegase_0.05_hexagon_32.png}
        \label{fig:best_obj_val:DCOPF:1354_pegase}
    }
    \subfloat[1354 Pegase 1\% ]{
        \includegraphics[width=0.33\columnwidth]{figs/BestObjVal_vs_time/pgd_obj_curve_1354_pegase_0.06_hexagon_32.png}
        \label{fig:best_obj_val:DCOPF:1354_pegase}
    }
    \subfloat[1354 Pegase 2\% ]{
        \includegraphics[width=0.33\columnwidth]{figs/BestObjVal_vs_time/pgd_obj_curve_1354_pegase_0.07_hexagon_32.png}
        \label{fig:best_obj_val:DCOPF:1354_pegase}
    }
    \subfloat[1354 Pegase 5\% ]{
        \includegraphics[width=0.33\columnwidth]{figs/BestObjVal_vs_time/pgd_obj_curve_1354_pegase_0.1_hexagon_32.png}
        \label{fig:best_obj_val:DCOPF:1354_pegase}
    }
    \subfloat[1354 Pegase 10\% ]{
        \includegraphics[width=0.33\columnwidth]{figs/BestObjVal_vs_time/pgd_obj_curve_1354_pegase_0.15_hexagon_32.png}
        \label{fig:best_obj_val:DCOPF:1354_pegase}
    }
    \subfloat[1354 Pegase 20\% ]{
        \includegraphics[width=0.33\columnwidth]{figs/BestObjVal_vs_time/pgd_obj_curve_1354_pegase_0.25_hexagon_32.png}
        \label{fig:best_obj_val:DCOPF:1354_pegase}
    }
    \mt{I would only keep 300+2\% and 300+10\% to illustrate that 1) Gurobi+bilevel may reject the warm-start, and 2) compact is the only one that ever manages to outperform PGA. All other instances are either "solved," or no significant difference. We could keep 300+5\% to indicate that 3) sometimes we can improve on PGA and 4) smaller input domain can yield better primal solutions faster. This last observation could be related to the input domain partitioning strategy for PGA.}
    \caption{Best objective value along time}
    \label{fig:best_obj_val_along_time:DCOPF}
\end{figure*}

\begin{table}[!t]
    \centering
    \caption{Best primal objective value achieved by each method. Each number is the geometric mean over 5 random seeds.}
    % \wc{New results updated 01/20}
    \mt{We should highlight that for hard instances (300 and 1354), Gurobi barely improves upon the PGA solution. In addition, for the 300-bus instances with 0\% -- 2\% noise, PGA appears to find a close-to-optimal solution.}
    \label{tab:primal_performanc}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{lrrrrrrr}
        \toprule
            &
            & \multicolumn{2}{c}{Heuristic}
            & \multicolumn{2}{c}{Compact}
            & \multicolumn{2}{c}{Bilevel}\\
        \cmidrule(lr){3-4}
        \cmidrule(lr){5-6}
        \cmidrule(lr){7-8}
        System & Noise (\%) &  Nom. & PGA & Nom & PGA & Nom & PGA\\
        \midrule
        57 
        & 0 & 45.08 & 127.36 & 141.36 & 141.36 & 141.36 & 141.36 \\
         & 1 & 45.08 & 137.35 & 142.29 & 142.29 & 142.29 & 142.29 \\
         & 2 & 45.08 & 143.70 & 151.54 & 151.54 & 151.54 & 151.54 \\
         & 5 & 45.08 & 171.53 & 179.12 & 179.12 & 179.12 & 179.12 \\
         & 10 & 45.08 & 175.89 & 432.20 & 432.21 & 432.20 & 432.21 \\
         & 20 & 45.08 & 1527.72 & 3837.33 & 3837.33 & 3837.33 & 3837.33 \\
        \midrule
        118   
        & 0 & 181.92 & 752.29 & 6216.97 & 6216.97 & 6216.97 & 6216.97 \\
         & 1 & 181.92 & 4615.37 & 7917.56 & 7917.56 & 7917.56 & 7917.56 \\
         & 2 & 181.92 & 4615.37 & 9607.68 & 9607.68 & 9607.68 & 9607.68 \\
         & 5 & 181.92 & 4615.37 & 14329.88 & 14329.87 & 14329.86 & 14329.86 \\
         & 10 & 181.92 & 5448.69 & 68556.32 & 68556.32 & 68556.32 & 68556.32 \\
         & 20 & 181.92 & 6048.77 & 69109.46 & 69109.46 & 69109.46 & 69109.51 \\
        \midrule
        300  
         & 0 & 4174.34 & 544923.75 & 546038.13 & 546038.13 & 546038.15 & 546038.55 \\
         & 1 & 4174.34 & 562348.32 & 564263.39 & 564263.44 & 564263.38 & 564263.40 \\
         & 2 & 4174.34 & 572166.01 & 572464.17 & 572464.17 & 572464.17 & 572460.26 \\
         & 5 & 4174.34 & 572166.01 & 651163.59 & 651163.38 & 651163.82 & 651163.54 \\
         & 10 & 4174.34 & 572166.01 & 596983.07 & 596983.90 & 466762.90 & 582808.43 \\
         & 20 & 4174.34 & 572166.01 & 582808.23 & 582808.47 & 410189.68 & 582808.47 \\
        \midrule
        1354 
         & 0 & 7323.96 & 380673.60 & 360031.97 & 380757.88 & 94216.80 & 380757.91 \\
         & 1 & 7323.96 & 399441.04 & 365497.51 & 399579.63 & 84443.61 & 399579.59 \\
         & 2 & 7323.96 & 403725.74 & 369678.23 & 406165.38 & 50115.73 & 406164.66 \\
         & 5 & 7323.96 & 403725.74 & 371524.52 & 406164.74 & 54315.20 & 406164.55 \\
         & 10 & 7323.96 & 571252.51 & 353196.16 & 571715.99 & 46631.55 & 571715.59 \\
         & 20 & 7323.96 & 571252.51 & 359722.30 & 578732.15 & 49521.07 & 578550.40 \\
         \bottomrule
    \end{tabular}
    }
    \mt{\textbf{Take-away from this table}: passing PGA warm-start to Gurobi always yields better primal solutions that passing nominal warm-start. Important note: the bilevel formulation will sometimes reject the warm-start because Gurobi cannot complete the (bilevel-feasible) solution within its work limits; this never happens with our compact formulation.}
\end{table}

}\fi

% \begin{table*}[!t]
% \centering
% \caption{Dual Bound (Upper Bound) Comparison of Single-Level and Bi-Level Formulations for the DCOPF Problem on 300\_ieee Network with Warm Start (WS) and without Warm Start (NO WS)}
% \begin{tabular}{lllll}
% \toprule
% $\pm$ XX \% &  single\_level (WS) &   single\_level (No WS) &     bi\_level\_milp (WS) & bi\_level\_milp (No WS) \\
% \midrule
% 1 &  \textbf{5809.51} &               6298.80 &              $\infty$ &             $\infty$ \\
% 2 &        9049961.41 &            5000181.28 &           11205370.12 &  \textbf{4932032.92} \\
% 3 &       18433219.75 &           13920908.72 &  \textbf{12941647.51} &          13501311.10 \\
% 5 &       35256775.06 &  \textbf{30082043.81} &           31701749.57 &          31571032.95 \\
% 10  &       50552696.36 &  \textbf{46349216.12} &           51534404.54 &          50743281.79 \\
% 12 &       55015961.89 &  \textbf{52426954.01} &           55223073.48 &          55403895.89 \\
% 15 &       62876123.16 &  \textbf{58523622.59} &           60477410.76 &          60570632.26 \\
% 20  &       72342460.43 &  \textbf{67800167.87} &           69152869.74 &          69646425.06 \\
% \bottomrule
% \end{tabular}
% \end{table*}

% \begin{table*}[!t]
% \centering
% \caption{Primal Bound (Lower Bound) Comparison of Single-Level and Bi-Level Formulations for the DCOPF Problem on 300\_ieee Network with Warm Start (WS) and without Warm Start (NO WS)}
% \mt{Those numbers are hard to understand out of the box. Report scaled optimality gap, i.e., divide the absolute gap by the objective value of the ED with nominal load. The current numbers look ginormous.}
% \begin{tabular}{lllll}
% \toprule
% $\pm$ XX \% &    single\_level (WS) & single\_level (No WS) & bi\_level\_milp (WS) & bi\_level\_milp (No WS) \\
% \midrule
% 1 &             2928.37 &    \textbf{2938.98} &           $-\infty$ &              $-\infty$ \\
% 2 &   \textbf{36589.56} &            24623.09 &          33347.71 &              $-\infty$ \\
% 3 &   \textbf{61166.65} &            46087.42 &           $-\infty$ &              $-\infty$ \\
% 5 &  \textbf{109406.82} &             $-\infty$ &           $-\infty$ &              $-\infty$ \\
% 10 &  \textbf{278395.56} &             $-\infty$ &           $-\infty$ &              $-\infty$ \\
% 12 &  \textbf{368104.75} &             $-\infty$ &           $-\infty$ &              $-\infty$ \\
% 15 &  \textbf{463266.50} &             $-\infty$ &           $-\infty$ &              $-\infty$ \\
% 20  &  \textbf{571453.35} &             $-\infty$ &           $-\infty$ &              $-\infty$ \\
% \bottomrule
% \end{tabular}
% \end{table*}


\subsection{Optimality Verification for Knapsack}
\subsubsection{Experiment Setup}
The optimality verification for Knapsack proxies is evaluated knapsack problems with different items.
The data is generated by perturbing the total capacity of knapsack and the item values, where the scaler of the total capacity $l$ and the item values $\vv$ are sampled from the uniform distribution $U[80\%, 120\%]$. More information of the knapsack proxies is detailed in the Appendix \ref{appendix:knapsack}.

The input domain is defined as:
\begin{align*}
    &\gX = \{\alpha\cdot l,\mBeta\cdot \vv| 1 - u\leq \alpha \leq 1 + u, 1- \mathbf{u} \leq \mBeta \leq 1+\mathbf{u}\},
\end{align*}
where $u$ control the size of the input domain.


\subsubsection{Performance of Exact Verification}

\begin{table}[!t]
    \centering
    \caption{Optimality Verification for Knapsack}
    \label{tab:optimality:knapsack}
    \begin{tabular}{lrrr}
        \toprule
        \#items & \%$u$ & gap (\%) & time (s) \\
        \midrule
        10 
         & 1 & 0.0 & 0.4 \\
         & 5 & 0.0 & 0.4 \\
         & 10 & 0.0 & 0.4 \\
         & 20 & 0.0 & 0.7 \\
        \midrule
        50 
         & 1 & 0.0 & 89.1 \\
         & 5 & 0.0 & 117.3 \\
         & 10 & 0.0 & 642.8 \\
         & 20 & 142.0 & t.o. \\
        \midrule
        80 
         & 1 & 0.0 & 1928.3 \\
         & 5 & 0.0 & 5997.8 \\
         & 10 & 230.0 & t.o. \\
         & 20 & 1350.0 & t.o. \\
        % \midrule
        % 100 
        %  & 1 & 0.0 & 497.8 \\ 
        %  & 5 & 140.0 & t.o. \\ 
        %  & 10 & 1223.0 & t.o. \\ 
        %  & 20 & 1558.0 & t.o. \\ 
        \bottomrule
    \end{tabular}\\
    \footnotesize{$^{*}$ Solved with 10 threads and time limits of 6 hours.}
    \vspace{-1em}
\end{table}

One compelling use case of the compact formulation is to verify proxies on approximating non-convex optimizations.
As shown in Table \ref{tab:optimality:knapsack}, the compact formulation can verify different proxies trained on Knapsack instances with different numbers of items.
It proves the compact formulation can verify broader classes of optimization problems than the bilevel counterparts.

\iffalse{
\begin{table*}[!t]
    \centering
    \caption{Optimality Verification for Knapsack}
    \wc{TODO: updated}
    \label{tab:optimality:knapsack}
    \begin{tabular}{lrrrrrrrr}
        \toprule
        \#items & noise (\%) & \#continous$^{*}$ & \#integer$^{*}$ & \#binary$^{*}$ & ub & lb & gap (\%) & time (s) \\
        \midrule
        10 & 1 & 50 & 12 & 12 & 0.0 & 0.0 & 0.0 & 0.4 \\
        10 & 5 & 50 & 12 & 12 & 0.0 & 0.0 & 0.0 & 0.4 \\
        10 & 10 & 63 & 19 & 19 & -84.7 & -84.7 & 0.0 & 0.4 \\
        10 & 20 & 111 & 100 & 95 & -93.7 & -93.7 & 0.0 & 0.7 \\
        \midrule
        50 & 1 & 3879 & 4922 & 4877 & -59.7 & -59.7 & 0.0 & 89.1 \\
        50 & 5 & 4001 & 5127 & 5082 & -66.0 & -66.0 & 0.0 & 117.3 \\
        50 & 10 & 4061 & 5318 & 5273 & -74.4 & -74.4 & 0.0 & 642.8 \\
        50 & 20 & 4368 & 5483 & 5437 & -81.1 & -196.5 & 142.0 & 63171.0 \\
        \midrule
        80 & 1 & 10339 & 10213 & 10137 & -41.5 & -41.5 & 0.0 & 1928.3 \\
        80 & 5 & 11799 & 12858 & 12779 & -70.8 & -70.8 & 0.0 & 5997.8 \\
        80 & 10 & 12009 & 13137 & 13058 & -74.4 & -539.5 & 626.0 & 63125.0 \\
        80 & 20 & 12125 & 13211 & 13132 & -92.6 & -1654.3 & 1687.0 & 63044.0 \\
        \midrule
        100 & 1 & 19391 & 24700 & 24601 & -56.6 & -56.6 & 0.0 & 4207.8 \\
        100 & 5 & 19373 & 24619 & 24520 & -80.9 & -190.2 & 140.0 & 63288.0 \\
        100 & 10 & 19351 & 24475 & 24376 & None & -1549.2 & None & 62659.0 \\
        100 & 20 & 19533 & 24576 & 24477 & -88.1 & -1460.6 & 1558.0 & 63061.0 \\
        \bottomrule
    \end{tabular}\\
    \footnotesize{$^{*}$After presolving. Solved with 10 threads.}
    \vspace{-1em}
\end{table*}
\fi


